A restricted four-body problem for the eight figure choreography

In this work we introduce a planar restricted four-body problem where a massless particle moves under the gravitational influence due to three bodies following the eight figure choreography, and we explore some symmetric periodic orbits of this system which turns out to be non autonomous. We demonstrate that certain families of involutions are reversing symmetries of certain N-body problem. We consider a particular case of such families of reversing symmetries and we use it to study both theoretically and numerically certain type of symmetric periodic orbits of this system. The symmetric periodic orbits (initial conditions) were determined by means of solving some boundary value problems.

==> engnames.tex <==
%
% engnames.tex 20.12.2006
%
\makeatletter
\def\contentsname{Contents}
\def\notesname{Notes}
\def\partname{Part}
\def\tocname{Contents}
\def\lofname{List of Figures}
\def\lotname{List of Tables}
\def\refname{REFERENCES}
\def\indexname{Index}
\def\figurename{Fig.}
\def\figuresname{Figures}%
\def\tablename{Table}
\def\tablesname{Tables}%
\def\abstractname{Abstract}
\def\appendixesname{Appendixes}%
\def\appendixname{Appendix}%
\def\acknowledgmentsname{Acknowledgments}
\def\journalname{??}
\def\copyrightname{??}
\def\andname{and}
\def\@pacs@name{MSC2010~numbers:}%
\def\@ydk@name{“„Љ~}%
\def\@keywords@name{Keywords:}%
\def\ppname{pp}
\def\numbername{number}
\def\volumename{volume}
\def\Dated@name{dated: }%
\def\Received@name{received }%
\def\Revised@name{in final form,~}%
\def\Accepted@name{accepted }%
\def\Published@name{published }%
\def\Presented@name{}%
%! 08.11.2006
\def\proofname{Proof}
\def\theoremname{Theorem}
\def\lemmaname{Lemma}
\def\propositionname{Proposition}
\def\assertionname{Assertion}
\def\corollaryname{Corollary}
\def\conjecturename{Conjecture}
\def\definitionname{Definition}
\def\remarkname{Remark}
\def\examplename{Example}
%!!
\makeatother
% ‘Ўа®б бзҐвзЁЄ®ў
\makeatletter
\setcounter{teo}{0}
\setcounter{teon}{0}
\setcounter{lem}{0}
\setcounter{lemn}{0}
\setcounter{prp}{0}
\setcounter{prpn}{0}
\setcounter{ass}{0}
\setcounter{assn}{0}
\setcounter{cor}{0}
\setcounter{corn}{0}
\setcounter{hyp}{0}
\setcounter{hypn}{0}
\setcounter{proof}{0}
\setcounter{proofn}{0}
\setcounter{exa}{0}
\setcounter{exan}{0}
\setcounter{dfn}{0}
\setcounter{dfnn}{0}
\setcounter{rem}{0}
\setcounter{remn}{0}
\setcounter{problem}{0}
\setcounter{problemn}{0}
\setcounter{notat}{0}
\setcounter{notatn}{0}
\makeatother
\endinput


==> jpack_e.tex <==
%%
%% This is file  `jpack_e.tex',  Strelkov S.A.  20.12.2006
%%
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsfonts}
%\usepackage{oldlfont} %%% Љ®­д«ЁЄвгҐв б bm.sty
\usepackage{mathtext}
\usepackage[T2A,OT1]{fontenc}
\usepackage[cp1251]{inputenc}
\usepackage[russian,english]{babel}
%\usepackage{literat}
\usepackage{pifont}
\usepackage{bm}
\usepackage{array}
\usepackage{dcolumn}
\usepackage{hhline}
\usepackage{multirow}
\usepackage{graphicx}
\usepackage{epsfig,color}
\usepackage{rotating}
\usepackage{srcltx_p}
\usepackage{calc}
\usepackage{tabularx}
\usepackage{afterpage}
\usepackage{ifthen}
\usepackage{caption2n}
\usepackage{substr}
%\usepackage{minitoc} 
\usepackage{psfrag}
\usepackage[all]{xy}
\usepackage{mathrsfs}
%\usepackage{supertabular}
\RequirePackage{soul}
\RequirePackage[amsmath]{ntheorem}
\RequirePackage{verbatim}
%
\theoremseparator{.}
\theoremindent 0pt
\theorempreskipamount 6pt plus2pt minus2pt
\theorempostskipamount 6pt plus2pt minus2pt
%
\RequirePackage{enumerate}
\makeatletter
\setcaptionwidth{\linewidth}
\renewcommand{\captionlabeldelim}{.~}
\renewcommand{\captionlabelfont}{\bfseries}
\renewcommand{\captionfont}{\footnotesize}
\renewcommand \thefigure{\@arabic\c@figure}
\renewcommand \thetable{\@arabic\c@table}
\renewcommand{\arraystretch}{1.5}
\setlength{\extrarowheight}{2pt}
\setlength{\extratabsurround}{2pt}
%%% Љ Є ў YADR.CLS
\renewcommand{\topfraction}{.90}
\renewcommand{\dbltopfraction}{.90}
\renewcommand{\bottomfraction}{.90}
\renewcommand{\textfraction}{0.10}
\renewcommand{\floatpagefraction}{0.90}
\renewcommand{\dblfloatpagefraction}{0.90}
\setcounter{topnumber}{4}
\setcounter{bottomnumber}{2}
\setcounter{totalnumber}{6}
%
\newcommand{\PreserveBackslash}[1]{\let\temp=\\#1\let\\=\temp}
\let\PBS=\PreserveBackslash
\def\settabpars#1#2#3{\vskip#1mm \tabcolsep=#2pt \def\arraystretch{#3}}
\newdimen\tabwidth\newdimen\tbwdth
\newcommand{\stretchtab}[2][1.0]{\setbox0=\hbox{\tabcolsep=0sp\ignorespaces#2}
          \setbox1=\hbox{\tabcolsep=1sp\ignorespaces#2}
          \tabwidth=#1\hsize \advance\tabwidth by -\wd0
          %\multiply\tabwidth by 1
          \tbwdth=\wd1\advance\tbwdth by -\wd0
          \divide\tabwidth by \tbwdth
          \tabcolsep=\tabwidth #2}
\newcommand\figcaption{\def\@captype{figure}\caption}
% 26.07.2006 \newcommand\tabcaption{\def\@captype{table}\caption}
\newcommand\tabcaption{\let\captionfont\small\def\@captype{table}\caption}
\renewcommand*\caption@@@normal{%
\parfillskip0pt plus 2fil%
  \caption@label\captiontext\par}
\newcaptionstyle{nonumber}{%
  \usecaptionmargin%
  \captionfont%
  \onelinecaption%
    {{\parbox[t]{\realcaptionwidth}{\parfillskip0pt plus 2fil\captiontext}}}%
    {\parfillskip0pt plus 2fil\captiontext}
}%
\newcommand{\commes}[1]{#1}
%\newcommand{\commes}[1]{\relax}
\def\place@bibnumber@inl#1{#1.}%
\flushbottom
\def\refitem#1{\relax}
%\def\refitem#1{\ifthenelse{\boolean{hmode}}{\protect\newline{}}{}\textbackslash{}refitem\{\hbox{\bfseries{}\itshape{}#1}\}\ifthenelse{\boolean{hmode}}{\protect\linebreak{}}{}}

\def\qedsymbol{\square}
\def\qed{\ifmmode\let\next\eqnqed\else
    \let\next\textqed\fi\next}
\def\eqnqed{\relax\eqno{\raisebox{-2mm}{\qedsymbol}}\ignorespaces}
\def\textqed{{\unskip\nobreak\hfil\penalty50\hskip1em\null\nobreak\hfil
    $\qedsymbol$\parfillskip\z@\finalhyphendemerits0\smallbreak\par}}
\def\p@subsubsection{}
\def\p@subsection{}
\def\p@section{}
\let\mtcSfont=\mtcSSfont
\def\l@section#1#2{%
 \addpenalty{1000}%
 \addvspace{0.4em plus 5\p@}%
 \@tempdima 2em %
 \begingroup\leftskip=-2em
  \parindent \z@ \rightskip \@tocrmarg
  \parfillskip -\rightskip
  \leavevmode %
  \advance\leftskip\@tempdima %
  \hskip -2em %
  #1\nobreak\hfil \nobreak\hb@xt@\@pnumwidth{\hss #2}\nopagebreak\par
 \endgroup
}%
\def\l@subsection#1#2{%
 \addpenalty{2000}%
 \addvspace{0em plus 1\p@}%
 \@tempdima=3em %
 \begingroup
  \leftskip=0em
  \parindent 0em \rightskip \@tocrmarg
  \parfillskip -\rightskip
  \leavevmode
  \advance\leftskip\@tempdima %
  \hskip -\leftskip %
  #1\nobreak\hfil \nobreak\hb@xt@\@pnumwidth{\hss #2}\nopagebreak\par
 \endgroup
}%
%\def\l@subsection{\@dottedtocline{2}{0em}{2.5em}}
\def\theequation{\arabic{section}.\arabic{equation}}
\@addtoreset{equation}{section}

\gdef\th@nonumberplain{%
  \def\@begintheorem##1##2{%
      \item[\hskip\labelsep \theorem@headerfont ##1.]}%
  \def\@opargbegintheorem##1##2##3{%
     \item[\hskip\labelsep \theorem@headerfont ##1\ {\upshape(}##3\/{\upshape)}.]}}

\renewcommand{\labelenumi}{$\theenumi.$}
\def\const{{\rm const}}

\makeatother
\endinput


==> maikdoi.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%             This is maikdoi.tex  V 1.2 22.10.2009
%
% ЋЈа ­ЁзҐ­ЁҐ: ¬®¦­® а Ў®в вм в®«мЄ® б ISSN б®бв®пйЁ¬ Ё§ жЁда;
%              ¬®¦­® § ¤ ў вм \JournalISSNCode(1234-567X)
%              Ё«Ё \JournalCode(X2345671); ­Ґв Їа®ўҐаЄЁ Є®­ва®«м­®© бг¬¬л ISSN.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\ProvidesFile{maikdoi.tex}
              [2009/10/23 v1.2
       add-on for MAIK document class revtex4n]
\typeout{revtex4n Class enhancement: maikdoi.tex for DOI}
%
\makeatletter
%
\def\JournalISSNnumber#1#2#3#4#5#6#7#8#9\@fin{\gdef\@JournalISSNnumber{#1#2#3#4#6#7#8#9}}
\expandafter\JournalISSNnumber\@JournalISSNCode\@fin
\typeout{JournalISSNnumber=\@JournalISSNnumber}
% macros to get and set the basic informations
%\def\journalnumber#1{\xdef\journ@lnumber{\padt@eight@digits{#1}}%
\def\journalnumber#1{\xdef\journ@lnumber{#1}%
%\checksize{journalnumber}8\journ@lnumber{99999999}%
}%
%\let\journ@lnumber=\empty
%
\def\ShortYear#1#2#3#4\@fin{\gdef\@ShortYear{#3#4}}
\expandafter\ShortYear\@TransYearOfIssue\@fin
\typeout{ShortYear=\@ShortYear}
\def\DOIyear#1{\xdef\DOI@year{\padt@two@digits{#1}}\checksize{DOIyear}2\DOI@year{99}}%
%
\def\DOIpsniy#1{\xdef\DOI@psniy{\padt@two@digits{#1}}% psniy - PublicationSerialNumberInYear
\checksize{DOIpsniy}2\DOI@psniy{99}}%
%
\def\DOIartnumber#1{\xdef\DOI@artnumber{\padt@three@digits{#1}}%
\checksize{DOIartnumber}3\DOI@artnumber{999}}
\def\DOI@artnumber{0}
%
\def\doitext#1{\xdef\doit@xtpref{#1}}
%
% a helpful hand of macros
\newif\if@wrongformat \@wrongformatfalse
%
\def\checksize#1#2#3#4{\ifnum#3>#4\PackageError{DOI2module}%
{Numeric value for "#1" to large!\MessageBreak
"#3" specified, but only #2 digits allowed}{Check your input!}
\@wrongformattrue \fi}
%
\newcount\modarg
\newcount\modmod
\newcount\tmp
\def\modulo{\tmp=\modarg\divide\modarg by\modmod\multiply\modarg
by\modmod\multiply\modarg by-1\global\advance\modarg by\tmp}
%
\def\padt@two@digits#1{\ifnum#1<10 0\fi\number#1}%
\def\padt@three@digits#1{\ifnum#1<100 0\fi%
\ifnum#1<10 0\fi\number#1}%
\def\padt@four@digits#1{\ifnum#1<1000 0\fi\ifnum#1<100 0\fi%
\ifnum#1<10 0\fi\number#1}%
\def\padt@five@digits#1{\ifnum#1<10000 0\fi\ifnum#1<1000 0\fi\ifnum#1<100 0\fi%
\ifnum#1<10 0\fi\number#1}%
\def\padt@eight@digits#1{\ifnum#1<1000000 0\fi\ifnum#1<1000000 0\fi\ifnum#1<100000 0%
\fi\ifnum#1<10000 0\fi\ifnum#1<1000 0\fi\ifnum#1<100 0\fi%
\ifnum#1<10 0\fi\number#1}%
%\def\setjahr#1{\xdef\jahr{#1}}
% @pii_digits_weights = (53,47,43,41,37,31,29,23,19,17,13,7,5,3,2);
\def\teilissn#1#2#3#4#5#6#7#8\@fin{%
\if#1X\modarg=10\relax\else\modarg=#1\relax\fi\multiply\modarg by53\advance\tmp by\modarg%
\if#2X\modarg=10\relax\else\modarg=#2\relax\fi\multiply\modarg by47\advance\tmp by\modarg%
\if#3X\modarg=10\relax\else\modarg=#3\relax\fi\multiply\modarg by43\advance\tmp by\modarg%
\if#4X\modarg=10\relax\else\modarg=#4\relax\fi\multiply\modarg by41\advance\tmp by\modarg%
\if#5X\modarg=10\relax\else\modarg=#5\relax\fi\multiply\modarg by37\advance\tmp by\modarg%
\if#6X\modarg=10\relax\else\modarg=#6\relax\fi\multiply\modarg by31\advance\tmp by\modarg%
\if#7X\modarg=10\relax\else\modarg=#7\relax\fi\multiply\modarg by29\advance\tmp by\modarg%
\if#8X\modarg=10\relax\else\modarg=#8\relax\fi\multiply\modarg by23\advance\tmp by\modarg}
\def\teilyear#1#2\@fin{%
\modarg=#1\relax\multiply\modarg by19\advance\tmp by\modarg%
\modarg=#2\relax\multiply\modarg by17\advance\tmp by\modarg}
\def\teilpsniy#1#2\@fin{%
\modarg=#1\relax\multiply\modarg by13\advance\tmp by\modarg%
\modarg=#2\relax\multiply\modarg by7\advance\tmp by\modarg}
\def\teilartnumber#1#2#3\@fin{%
\modarg=#1\relax\multiply\modarg by5\advance\tmp by\modarg%
\modarg=#2\relax\multiply\modarg by3\advance\tmp by\modarg%
\modarg=#3\relax\multiply\modarg by2\advance\tmp by\modarg}
%
% check for all required elements
\def\checkrequirements{
\if!\journ@lnumber!\typein[\answer]{^^JMissing 5-digit
journalnumber for the DOI, please specify:}\journalnumber\answer\fi
%
\ifnum\OF@year=0\typein[\answer]{^^JMissing 4-digit year for the OF
date, please specify:}\OFyear\answer\fi
%
\ifnum\DOI@year=0\typein[\answer]{^^JMissing 4-digit year for the DOI,
please specify:}\DOIyear\answer\fi
{\modarg=\DOI@year\relax\modmod=1000\relax\modulo
\expandafter\setjahr{\padt@three@digits\modarg}}
%
\if!\the\DOI@msnr!\typein[\answer]{^^JMissing 4-digit
manuscript number for the DOI, please specify:}\DOImsnr\answer\fi}
%
% make the package verbose
\def\showDOIargs{%
\typeout{^^JList of arguments for this DOI2 generation
^^J==========================================
^^JDOI-prefix :\space\maikpraefix
^^JISSN number:\space\journ@lnumber
^^JDOI-year\space\space\space:\space\DOI@year
^^JIn-Year-No.:\space\DOI@psniy
^^JArticle-No.:\space\DOI@artnumber
^^J==========================================}}
%
% perform the calculation
\def\DOIt{\if@wrongformat
   \typeout{Wrong format of at least one required value,^^Jno
            DOI could be generated.^^J}%
\else
   \edef\doit@xtcode{%
   \maikpraefix\journ@lnumber\DOI@year\DOI@psniy\DOI@artnumber}%
   \tmp=0\relax%
   \expandafter\teilissn\journ@lnumber\@fin%
   \expandafter\teilyear\DOI@year\@fin%
   \expandafter\teilpsniy\DOI@psniy\@fin%
   \expandafter\teilartnumber\DOI@artnumber\@fin%
   \modarg=\tmp\modmod=11\relax\modulo
   \ifnum\modarg<10\edef\checksum{\the\modarg}\else\edef\checksum{X}%
   \fi
   \edef\doit@xtcode{\doit@xtcode\checksum}
   \edef\doit@xt{\doit@xtpref\doit@xtcode}
   \showDOIargs
   \typeout{Calculated DOI:\space\space\doit@xtcode
   ^^J^^JVerbose:^^J\doit@xt^^J}
\fi
}
%
% set the defaults - the basics at least
%\def\springerpraefix{10.1007/s}
%!\def\maikpraefix{10.1134/S}
\doitext{\relax}%
%! 22.10.2009
\def\OnlineFirstDOI#1#2{\def\doit@xtcode{#1}%
\def\@onlinefirstdoi{#1}%
\def\@onlinefirstfilename{#2}%
\@booleantrue\onlinefirstdoi@sw%
\ifthenelse{\equal{\@nameincfi}{#2}}{%
\addtocounter{doiartnumber}{-\@ne}
}%
{\class@err{ ^^J^^J
\space\space \noexpand\OnlineFirstDOI{#1}{#2}^^J
\space\space Name Online First file:  #2^^J
\space\space Includepaper file name: \@nameincfi^^J
\space\space Not equal}%
}%
}%
%!!
%
\journalnumber{\@JournalISSNnumber}
\typeout{journalnumber=\journ@lnumber}
\DOIyear{\@ShortYear}
\typeout{DOIyear=\DOI@year}
\DOIpsniy{\@PublicationSerialNumberInYear}
\typeout{DOIpsniy=\DOI@psniy}
\makeatother
\endinput
%% End of file `maik.doi'

